INetCEP: In-Network Complex Event Processing for Information-Centric Networking

Emerging network architectures like Information-centric Networking (ICN) offer simplicity in the data plane by addressing named data. Such flexibility opens up the possibility to move data processing inside network elements for high-performance computation, known as in-network processing. However, existing ICN architectures are limited in terms of data plane programmability due to the lack of (i) in-network processing and (ii) data plane programming abstractions. Such architectures can benefit from Complex Event Processing (CEP), an in-network processing paradigm to efficiently process data inside the data plane. Yet, it is extremely challenging to integrate CEP because the current communication model of ICN is limited to consumer-initiated interaction that comes with significant overhead in a number of requests to process continuous data streams. In contrast, a change to producer-initiated interaction, as favored by CEP, imposes severe limitations for request-reply interactions. In this paper, we propose an in-network CEP architecture, INetCEP that supports unified interaction patterns (consumer- and producer-initiated). In addition, we provide a CEP query language and facilitate CEP operations while increasing the range of applications that can be supported by ICN. We provide an open-source implementation and evaluation of INetCEP over an ICN architecture, Named Function Networking, and two applications: energy forecasting in smart homes and a disaster scenario.

==> sections/designgoals.tex <==
\begin{comment}
\section{Design Goals}\label{sec:designgoals}
\mli{combine system model and design goals to be 1 column?}
\subsection{Unified Network Layer (Communication Model)}

push + pull design

\subsection{Ability to Express Complex Expressions (Query Model)}

\subsection{Query Decomposition, Distribution and Placement (Query Optimization and Placement)}
dealing with stateful operators - cache management
node discovery + distribution + placement
\end{comment}
